Dialog without Dialog Data: Learning Visual Dialog Agents from VQA Data

Can we develop visually grounded dialog agents that can efficiently adapt to new tasks without forgetting how to talk to people? Such agents could leverage a larger variety of existing data to generalize to new tasks, minimizing expensive data collection and annotation. In this work, we study a setting we call "Dialog without Dialog", which requires agents to develop visually grounded dialog models that can adapt to new tasks without language level supervision. By factorizing intention and language, our model minimizes linguistic drift after fine-tuning for new tasks. We present qualitative results, automated metrics, and human studies that all show our model can adapt to new tasks and maintain language quality. Baselines either fail to perform well at new tasks or experience language drift, becoming unintelligible to humans. Code has been made available at https://github.com/mcogswell/dialog_without_dialog

==> Dialog Without Dialog NeurIPS/result_tables/ablations.tex <==
{\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr}
\toprule
& Accuracy & Perplexity & Relevance & Diversity \\
\midrule
DWD (Ours)           &     0.81 &      2.57 &         0.89 &        0.86 \\
Fine Decoder         &     0.82 &      2.54 &         0.85 &        0.59 \\
Parallel Speaker     &     0.78 &      2.60 &         0.88 &        0.73 \\
Stage 1              &     0.72 &      2.60 &         0.91 &        0.48 \\
Stage 2.A            &     0.80 &      2.59 &         0.89 &        0.81 \\
Stage 2.B (Skip 2.A) &     0.80 &      2.53 &         0.85 &        0.62 \\
\bottomrule
\end{tabular}
}
}

==> Dialog Without Dialog NeurIPS/result_tables/curricula_comparison.tex <==

{
\newcommand{\num}[1]{\texttt{\footnotesize #1}}
\newcommand{\g}{\cellcolor{gray!10}}

\resizebox{\columnwidth}{!}{
\begin{tabular}{l l l l l c c c c}
\toprule
 & $z$ Structure & Loss & Curriculum & Speaker & Accuracy & Perplexity & Relevance & Diversity \\
\midrule
\g \num{1} & \g Discrete &\g ELBO & \g Stage 2.B & \g Fixed  &     \g 0.81 &      \g 2.57 &        \g 0.89 &       \g \textbf{0.86} \\
\num{2} &Discrete &ELBO & Stage 2 & Fine-tuned          &     \textbf{0.82} &      2.54 &         0.85 &        0.59 \\
\g \num{3} &\g Discrete &\g ELBO & \g Stage 2 &\g Parallel           &   \g  0.78 &    \g  2.60 &      \g   0.88 &     \g   0.73 \\
\num{4} &Discrete &ELBO & Stage 1 &Fixed           &     0.72 &      2.60 &         \textbf{0.91} &        0.48 \\
\g \num{5} &\g Discrete &\g ELBO & \g Stage 2.A & \g Fixed         &  \g   0.80 &    \g  2.59 &      \g   0.89 &    \g    0.81 \\
\num{6} &Discrete &ELBO & Stage 2 & Fixed           &     0.80 &      \textbf{2.53} &         0.85 &        0.62 \\
\g \num{7} &\g Continuous &\g ELBO & \g Stage 2.B &\g  Fixed         &   \g  0.75 &   \g  2.45 &      \g   0.66 &     \g   0.23 \\
\num{8} &Continuous & MLE & Stage 2.B & Fixed         &     0.78 &      4.27 &         0.83 &        4.33 \\
\bottomrule
\end{tabular}
}
}




%{\footnotesize
%\resizebox{\columnwidth}{!}{
%\begin{tabular}{lrrrr}
%\toprule
%& Accuracy & Perplexity & Relevance & Diversity \\
%\midrule
%DWD (Ours)           &     0.81 &      2.57 &         0.89 &        0.86 \\
%Fine Decoder         &     0.82 &      2.54 &         0.85 &        0.59 \\
%Parallel Speaker     &     0.78 &      2.60 &         0.88 &        0.73 \\
%Stage 1              &     0.72 &      2.60 &         0.91 &        0.48 \\
%Stage 2.A            &     0.80 &      2.59 &         0.89 &        0.81 \\
%Stage 2.B (Skip 2.A) &     0.80 &      2.53 &         0.85 &        0.62 \\
%\midrule
%Cont Stage 2.B         &     0.75 &      2.45 &         0.66 &        0.23 \\
%DWD (Ours)             &     0.81 &      2.57 &         0.89 &        0.86 \\
%Non-Var Cont Stage 2.B &     0.78 &      4.27 &         0.83 &        4.33 \\
%\bottomrule
%\end{tabular}
%}
%}

==> Dialog Without Dialog NeurIPS/result_tables/human_interactive.tex <==




{
\newcommand{\num}[1]{\texttt{\footnotesize #1}}

\resizebox{\columnwidth}{!}{
\begin{tabular}{l c c c c c}
\toprule
            & Accuracy \\
Round       & 1         & 2         & 3         & 4         & 5 \\
\midrule
\stageone{} & 20.8\%	&  25.0\%	&  22.9\%	&  35.4\%	&  22.9\% \\
\nonvar{}   & 26.5\%	&  53.1\%	&  51.0\%	&  46.9\%	&  44.9\% \\
\ours{}     & 18.4\%	&  61.2\%	&  53.1\%	&  65.3\%	&  69.4\%
\bottomrule
\end{tabular}
}

==> Dialog Without Dialog NeurIPS/result_tables/main_results_table.tex <==
\newcommand{\g}{\cellcolor{gray!10}}
\newcommand{\num}[1]{\texttt{\footnotesize #1}}


\renewcommand*{\arraystretch}{1.25}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c c l r r r r | c c l r r r r}
\toprule
 & & \small  & \small Accuracy $\uparrow$& \small Perplexity$\downarrow$ & \small Relevance $\uparrow$& \small Diversity$\uparrow$ & & & \small  & \small Accuracy $\uparrow$& \small Perplexity$\downarrow$ & \small Relevance $\uparrow$& \small Diversity$\uparrow$\\
 \midrule
 \multirow{3}{*}{\small \rotatebox{90}{\shortstack{\textbf{VQA} \\ 2 Contrast\\ 1 Round}}} &  
 \g \num{A1} & \g \stageone & \g0.73 &      \g2.62 &         \g0.87 &        \g0.50 & \multirow{3}{*}{\small \rotatebox{90}{\shortstack{\textbf{VQA} \\ 9 Random\\9 Rounds}}}
  & \g \num{D1} & \g \stageone & \g 0.18 &      \g 2.72 &         \g \textbf{0.77} &        \g 1.11 \\
  & \num{A2} & \nonvar & 0.71 &     10.62 &         0.66 &        \textbf{5.55} &  & \num{D2} & \nonvar &  \textbf{0.78} &     40.66 &       \textbf{0.77} &       \textbf{2.57} \\
  & \g\num{A3} & \g\ours & \g\textbf{0.82} & \g\textbf{2.6} & \g\textbf{0.88} & \g0.54 &   & \g \num{D3} & \g \ours & \g 0.53 &     \g \textbf{2.55} &       \g  0.75 &       \g 0.95 \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{3}{*}{\small \rotatebox{90}{\shortstack{\textbf{VQA} \\ 2 Contrast\\5 Rounds}}}
  & \num{B1} & \stageone & 0.67 &      2.62 &         0.87 &        0.50 & \multirow{3}{*}{\small \rotatebox{90}{\shortstack{\textbf{AWA} \\ 9 Random\\9 Rounds}}}
  & \num{E1} & \stageone &  0.47 &      2.49 &         \textbf{0.96} &        0.24 \\
  & \g\num{B2} & \g\nonvar & \g0.74 &     \g10.62 &         \g0.66 &       \g \textbf{5.55} &   & \g \num{E2} & \g \nonvar & \g 0.48 &     \g 12.56 &        \g 0.64 &        \g \textbf{2.21} \\

  & \num{B3} & \ours & \textbf{0.87} &      \textbf{2.60} &         \textbf{0.88} &        0.54 &   & \num{E3} & \ours & \textbf{0.74} & \textbf{2.41} &   \textbf{0.96} &  0.28 \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{3}{*}{\small \rotatebox{90}{\shortstack{\textbf{VQA} \\ 2 Random\\5 Rounds}}}
  & \g\num{C1} & \g\stageone & \g0.64 &    \g  \textbf{2.64} &     \g    0.75 & \g       1.73 & \multirow{3}{*}{\small \rotatebox{90}{\shortstack{\textbf{CUB} \\ 9 Random\\9 Rounds}}}
  & \g \num{F1} & \g \stageone & \g 0.36 &  \g    2.56 &         \g \textbf{1.00} &     \g   0.04 \\
  & \num{C2} & \nonvar & 0.86 &     16.95 &         0.62 &        \textbf{8.13} &   & \num{F2} & \nonvar &0.38 &     20.92 &         0.47 &        \textbf{2.16} \\
  &\g \num{C3} &\g \ours &\g \textbf{0.95} & \g     2.69 &    \g     \textbf{0.77} &     \g   2.34 &   &\g \num{F3} & \g \ours & \g \textbf{0.74} &     \g \textbf{2.47} &        \g \textbf{1.00} &    \g    0.04 \\
%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}}


==> Dialog Without Dialog NeurIPS/result_tables/mturk_question_comparison.tex <==
{\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr}
\toprule
                       & Neither & \stageone{} & \nonvar{} & \ours{}   \\
\midrule                          
\stageone{} vs \nonvar{} &  31.7\% &  48.1\%   &  20.2\%   &  --     \\
\stageone{} vs \ours{}     &  49.0\% &  26.2\%   &  --       &  24.8\% \\
\nonvar{} vs \ours{}     &  32.7\% &  --       &  17.9\%   &  49.4\% \\
\midrule
\stageone{} vs \nonvar{} &  19.6\% &  48.8\%   &  31.7\%   &  --     \\
\stageone{} vs \ours{}     &  25.0\% &  38.4\%   &  --       &  36.6\% \\
\nonvar{} vs \ours{}     &  22.0\% &  --       &  30.2\%   &  47.8\% \\
\bottomrule
\end{tabular}
}
}

==> Dialog Without Dialog NeurIPS/result_tables/mturk_question_comparison_fluency.tex <==
%% fluency raw counts
%\begin{tabular}{lrrrr}
%\toprule
%choice\_name &  baseline &  neither &   ours &  stage 1 \\
%exp\_pair                    &           &          &        &          \\
%\midrule
%exp15.0.1.0.0\_exp19.2.1.0.4 &     182.0 &    285.0 &    NaN &    433.0 \\ 900
%exp15.0.1.0.0\_exp20.2.2.0   &       NaN &    441.0 &  223.0 &    236.0 \\ 900
%exp19.2.1.0.4\_exp20.2.2.0   &     161.0 &    294.0 &  445.0 &      NaN \\ 900
%\bottomrule
%\end{tabular}


{\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr}
\toprule
                       & Neither & \stageone{} & \nonvar{} & \ours{}   \\
\midrule                          
\stageone{} vs \nonvar{} &  31.7\% &  48.1\%   &  20.2\%   &  --     \\
\stageone{} vs \ours{}     &  49.0\% &  26.2\%   &  --       &  24.8\% \\
\nonvar{} vs \ours{}     &  32.7\% &  --       &  17.9\%   &  49.4\% \\
\bottomrule
\end{tabular}
}
}

==> Dialog Without Dialog NeurIPS/result_tables/mturk_question_comparison_grounding.tex <==
%% grounding raw counts
%\begin{tabular}{lrrrr}
%\toprule
%choice\_name &  baseline &  neither &   ours &  stage 1 \\
%exp\_pair                    &           &          &        &          \\
%\midrule
%exp15.0.1.0.0\_exp19.2.1.0.4 &     285.0 &    176.0 &    NaN &    439.0 \\ 900
%exp15.0.1.0.0\_exp20.2.2.0   &       NaN &    225.0 &  329.0 &    346.0 \\ 900
%exp19.2.1.0.4\_exp20.2.2.0   &     272.0 &    198.0 &  430.0 &      NaN \\ 900
%\bottomrule
%\end{tabular}




{\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr}
\toprule
                       & Neither & \stageone{} & \nonvar{} & \ours{}   \\
\midrule                          
\stageone{} vs \nonvar{} &  19.6\% &  48.8\%   &  31.7\%   &  --     \\
\stageone{} vs \ours{}     &  25.0\% &  38.4\%   &  --       &  36.6\% \\
\nonvar{} vs \ours{}     &  22.0\% &  --       &  30.2\%   &  47.8\% \\
\bottomrule
\end{tabular}
}
}

==> Dialog Without Dialog NeurIPS/result_tables/vartype_comparison.tex <==
{\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr}
\toprule
& Accuracy & Perplexity & Relevance & Diversity \\
\midrule
Cont Stage 2.B         &     0.75 &      2.45 &         0.66 &        0.23 \\
DWD (Ours)             &     0.81 &      2.57 &         0.89 &        0.86 \\
Non-Var Cont Stage 2.B &     0.78 &      4.27 &         0.83 &        4.33 \\
\bottomrule
\end{tabular}
}
}

==> Dialog Without Dialog NeurIPS/sections/abstract.tex <==

Can we develop visually grounded dialog agents that can efficiently adapt to new tasks without
forgetting how to talk to people?
Such agents could leverage a larger variety of existing data to generalize to new task, 
minimizing expensive data collection and annotation.
In this work, we study a setting we call ``\textit{Dialog without Dialog}'', 
which requires agents
to develop visually grounded dialog models that can adapt to new tasks without
language level supervision.
By factorizing intention and language, our model minimizes
linguistic drift after fine-tuning for new tasks.
We present qualitative results, automated metrics, and human studies that
all show our model can adapt to new tasks and maintain language quality.
Baselines either fail to perform well at new tasks or experience language drift,
becoming unintelligible to humans. Code has been made available at: \href{https://github.com/mcogswell/dialog_without_dialog}{https://github.com/mcogswell/dialog\_without\_dialog}


==> Dialog Without Dialog NeurIPS/sections/acknowledgements.tex <==
i\section{Acknowledgements}

The Georgia Tech effort was supported in part by NSF, AFRL, DARPA, ONR YIPs, ARO PECASE, Amazon. The views and conclusions contained herein are those of the authors and should not be interpreted as necessarily representing the official policies or endorsements, either expressed or implied, of the U.S. Government, or any sponsor.


==> Dialog Without Dialog NeurIPS/sections/approach.tex <==
\section{Dialog Based Image Guessing Game}
% In this section we introduce our image guessing game and the bots that play the game.
% Later, \secref{sec:new_qbot} addresses the transfer required by the \dwd{} task.
% \jl{In this section, we first introduce the \dwd{} game definition with notations. Then we describe each modules in \abot{} and \qbot{} respectively. }

\subsection{Game Definition}
\label{sec:guessgame}

Our image guessing game proceeds one round at a time, starting at round $r = 1$ and running
for a fixed number of rounds of dialog $R$.
At round $r$, \qbot{} observes the pool of images $\mathcal{I} =\{I_1, \dots, I_P\}$ of size $P$, 
the history of question answer pairs $q_1, a_1, \dots q_{r-1}, a_{r-1}$, and placeholder representations $q_0, a_0$
that provide input for the first round. It generates a question
\begin{equation}
q_{r} =
    \mathtt{QBot.Ask}(\mathcal{I}, q_0, a_0, \dots q_{r-1}, a_{r-1}).
\end{equation}
Given this question, but not the entire dialog history, \abot{} answers based on the randomly selected target image $I_{\hat{y}}$ (not known to \qbot{}):
\begin{equation}
a_{r} =
    \mathtt{ABot.Answer}(I_{\hat{y}}, q_{r}).
\end{equation}
Once \qbot{} receives the answer from \abot{}, it makes a prediction $y_{r}$ guessing the target image:
\begin{equation}
y_{r} =
    \mathtt{QBot.Predict}(\mathcal{I}, q_0, a_0, \dots , q_{r}, a_{r})
\end{equation}
%
%where $\hat{y}$ is the ground truth for $y_{r}$ at every rounds.

\paragraph{Comparison to GuessWhich.}
Our Image Guessing game is inspired by GuessWhich game of \citet{visdial_rl}, and there are two subtle but important differences.
In GuessWhich, \qbot{} initially observes a caption describing \abot{}'s selected image and
must predict the selected image's features to retrieve it from a large, fixed pool of images it does not observe. 
First, the inclusion of the caption leaves little room for the dialog to add information~\cite{mironenco2017examining}, so we omit it.
Second, in our game a small pool of images is sampled for each dialog and \qbot{} directly predicts the target image given those choices.

\subsection{Modelling \abot{}}
\label{sec:abot}

In this work, we focus primarily on \qbot{} agent rather than \abot{}. 
We set \abot{} to be a standard visual question answering agent, specifically the Bottom-up Top-down \cite{bottomup_tricks} model; however, we do make one modification. \qbot{} may generate questions that are not well 
grounded in \abot{}'s selected image (though they may be grounded in other pool images) -- e.g. asking about a surfer when none exists.
To enable \abot{} to respond appropriately, we augment \abot{}'s answer space with a \texttt{Not Relevant} token. 
To generate training data for this token we augment every image with an additional randomly sampled question and
set \texttt{Not Relevant} as its target answer.
\abot{} is trained independently from \qbot{} on the VQAv2 dataset and then frozen.


\subsection{Modelling \qbot{}}
\label{sec:qbot}

We conceptualize \qbot{} as having three major modules.
The \emph{planner} encodes the state of the game to decide what to ask about.
The \emph{speaker} takes this intent and formulates the language to express it.
The \emph{predictor} makes target image predictions taking the dialog history into account.
We make fairly standard design choices here, then adapt this model for the \dwd{} task
in \secref{sec:dwd}.

\paragraph{Pool \& Image Encoding.}
We represent the $p$-th image $I_p$ of the pool as a set of $B$ bounding boxes such that 
$I^p_b$ is the embedding of the $b$-th box using the same Faster R-CNN~\cite{fasterrcnn} embeddings as
in \cite{bottomup}.
Note that we do not assume prior knowledge about the size or composition of the pool.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/qbot.pdf}
    \caption{\footnotesize{A single round of our \qbot{} which decomposes into the modules described in \secref{sec:qbot}. This factorization
    allows us to limit language drift while fine-tuning for task performance.}}
    \label{fig:qbot}
    \vspace{-10pt}
\end{figure} 

\paragraph{Planner.}
The planner's role is to encode the dialog context (image pool and dialog history) into representation $z^r$,
deciding what to ask about in each round. It also produces an encoding $h_r$ of the dialog history.
To limit clutter, we denote the question-answer pair at round $r$ as a `fact' $F_r = [q_r, a_r]$. 

\paragraph{Planner -- Context Encoder.}
Given the prior dialog state $h_{r-1}$, $F_{r-1}$, and image
pool $\mathcal{I}$, the context encoder performs 
hierarchical attention over images in $\mathcal{I}$ and object boxes in each image to identify image regions
that are most relevant for generating the next question. 
%
As we detail in Section \suppSectionArchitectureDetails{} of the supplement, $F_{r-1}$ and $h_{r-1}$ query the image to attend to relevant regions across the pool.
First a $P$ dimensional distribution $\alpha$ over images in the pool is produced
and then a $B$ dimensional distribution $\beta^p$ over boxes is produced for each image $p \in \{1, \ldots, P\}$.
The image pool encoding $\hat{v}_r$ at round $r$ is
\begin{align}
    \hat{v}_r = \sum_{p=1}^P \alpha_p \sum_{b=1}^B \beta^p_b I^p_b.
\end{align}
This combines the levels of attention and is agnostic to pool size.

\paragraph{Planner -- History Encoder.} 
To track the state of the game, the planner applies an LSTM-based history encoder that takes $\hat{v}_r$ and $F_{r-1}$ as input and produces an intermediate hidden state $h_{r}$.
%We denote this with a bar as it is further modified by the question policy before being passed to the next round. 
Here $h_{r}$ includes a compact representation of question intent and dialog history, helping provide a differentiable connection between the intent and final predictions through the dialog state. 

\paragraph{Planner -- Question Policy.}
The question policy transforms $h_{r}$ to this module's output $z^r$, which the speaker decodes into a question.
By default $z^r$ is equal to the hidden state $h_r$,
%the identity function (\ie, $z^r = h_{r}$),
but in \secref{sec:new_qbot} we show how %a different
%implementation 
a discrete representations 
can be used to reduce language drift.

\paragraph{Speaker.}
Given an intent vector $z^r$, the speaker generates a natural language question. Our speaker is a standard LSTM-based decoder with an initial hidden state equal to $z^r$. %or an embedding of $z^r$ (in \secref{sec:new_qbot}). 
% \todo{Some discussion of the vocabulary}

\paragraph{Predictor.}
The predictor uses the dialog context generated so far to guess the target image. It takes a concatenation $F = [F_1, \ldots, F_{r}]$ of fact embeddings and the dialog
state $h_{r}$ and computes an attention pooled fact $\hat{F}$ using $h_{r}$ as attention context.
Along with $h_{r}$, this is used to attend to salient image features then compute a distribution over images in the pool
using a softmax (see Algorithm 2 in the supplement for full details), allowing for
the use of cross-entropy as the task loss.
% This mechanism is again agnostic to the pool size, so 
Note that the whole model is agnostic to pool size.

\section{Dialog without Dialog}
\label{sec:dwd}

Aside from some abstracted details, the game setting and model presented in the previous section could be trained without any further information -- a pool of images could be generated, 
\abot{} could be assigned an image, the game could be rolled out for arbitrarily many rounds, and \qbot{} could be trained to predict the correct image given \abot{}'s answers. While 
this is an interesting research direction in its own right~\cite{ren20,chaabouni20,liang20}, there is an obvious shortcoming --
it would be highly improbable for \qbot{} to discover a fully functional language that humans can already understand.
Nobody discovers French. They have to learn it.

At the other extreme -- representing standard practice in dialog problems -- humans could be recruited to perform this image guessing game and provide dense supervision for what questions \qbot{} should ask to perform well at this specific task. However, this requires collecting language data for every new task. It is also intellectually dissatisfying for agents' knowledge of natural language to be so inseparably intertwined with individual tasks. After all, one of the greatest powers of language is the ability to use it to communicate about many different problems.

In this section, we consider a middle ground that has two stages. Stage 1 trains our agent on one task where training data already exists (VQA; \ie, single round dialog) and then 
stage 2 adapts it to carry out goal driven dialog (image guessing game) without further supervision. 

\subsection{Stage 1: Language Pre-training}
\label{sec:stage1}
%We want \qbot{}'s language to be interpretable -- in this paper we take that to mean
%it should be understandable by and semantically meaningful to humans,
%so it has to be something like a meaningful subset of a known human language. To pre-train the model to use interpretable human language, we design a supervised learning task for a single-round version of our game.

%\xhdr{Single-shot Question Answering Training.} 
We leverage the VQAv2~\cite{vqav2} dataset as our language source to 
learn how to ask questions that humans can understand. By construction, for each question in VQAv2 there exists at least one pair of images which are visually similar but have different ground truth answers to the same question.
Fortuitously, this resembles our dialog game -- the image pair is the pool, the question is guaranteed to be discriminative, and we can provide an answer depending on \abot{}'s selected image.
We view this as a special case of our game that is fully supervised but contains only a single round of dialog.
During stage 1 \qbot{} is trained to mimic the human question (via cross-entropy teacher forcing) and to predict the correct image given the ground truth answer.

For example, in the top left of \figref{fig:guesswhich} outlined in dashed green we show a pair of two bird images with the question ``What is in the bird's beak?'' from VQAv2.
Our agents engage in a single round dialog where \qbot{} asks that question and \abot{} provides the answer (also supervised by VQAv2).

\subsection{Stage 2: Transferring to Dialog}
\label{sec:new_qbot}

A first approach for adapting agents would be to
take the pre-trained weights from stage 1 and simply fine-tune for our full image guessing task.
However, this agent would face a number of challenges. It has never had to model multiple steps of a dialog.
Further, while trying to predict the target image there is little to encourage \qbot{} to continue producing intelligible language.
Indeed, we find our baselines do exhibit language drift.
We consider four modifications to address these problems.

%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.49\textwidth]{figures/elbo.pdf}
%    \caption{}
%    \label{fig:pretraining}
%\end{figure} 

\paragraph{Discrete Latent Intention Representation $z^r$.}
\label{sec:pre-training}
Rather than a continuous vector passing from the question policy to the speaker, we pass discrete vectors.
Specifically, we consider a representation composed of $N$ different $K$-way Concrete variables~\cite{concrete_distribution}.
Let $z^r_n \in \{1, \ldots, K\}$ and let the logits $l_{n,1}, \ldots, l_{n,K}$ paramterize the Concrete distribution $p(z^r_n)$.
We learn a linear transformation $W^z_n$ from the intermediate dialog state $h_{r}$ to produce these logits for each variable $n$:%
\begin{align}
    l_{n,k} &= \mathrm{LogSoftmax}\left(W^z_n h_{r} \right)_k \; \forall k \in \{1, \ldots, K\} \; \forall n \in \{1, \ldots, N\}
\end{align}
%
To provide input to the speaker, $z^r$ is embedded using a learned dictionary of embeddings.
In our case each variable in $z^r$ has a dictionary of $K$ learned embeddings.
The value of $z^r_n$ ($\in \{1, \ldots, K\}$) picks one of the embeddings
for each variable and the final representation simply sums over all variables:
%
\begin{align}
    e_z = \sum_{n=1}^{N} E_n(z^r_n).
\end{align}
%
\paragraph{VAE Pre-training.}
When using this representation for the intent, we train stage 1 by replacing the likelihood with an ELBO (Evidence Lower BOund) loss
as seen in Variational Auto-Encoders (VAEs)~\cite{vae} to
help disentangle intent from expression by
restricting information flow through $z^r$.
% TODO: correctly deal with the unspecified VAE and ELBO acronyms
We use the existing speaker module to decode $z^r$ into questions and train a new encoder
module to encode ground truth VQAv2 question $\hat{q}_1$ into conditional distribution $q(z^1 | \hat{q}_1, \mathcal{I})$ over $z^r$ at round 1.

For the encoder we use a version of the previously described context encoder from \secref{sec:qbot} that
uses the question $\hat{q}_1$ as attention query instead of $F_{r-1}$ and $h_{r-1}$ (which are not available in this context).
The resulting ELBO loss is
%
\begin{align}
    \mathcal{L} = 
    & E_{z^1 \sim q(z^1 | \hat{q}_1, \mathcal{I})}\left[ \log p(\mathtt{speaker}(z^1)) \right] +
        \frac{1}{N} \sum_{n=1}^{N} D_{KL}\left[ q(z^1_n | \hat{q}_1, \mathcal{I}) || \mathcal{U}(K) \right]
    \label{eq:elbo}
\end{align}
%
This is like the Full ELBO described, but not implemented, in \cite{rethink_zhao}.
The first term encourages the encoder to represent and the speaker to mimic the VQA question.
The second term uses the KL Divergence $D_{KL}$ to push the distribution of $z$ close to
the $K$-way uniform prior $\mathcal{U}(K)$, encouraging $z$ to ignore irrelevant information.
Together, the first two terms form an ELBO on the question likelihood
given the image pool~\cite{gumbel_softmax,kaiser18}.

\paragraph{Fixed Speaker.}
Since the speaker contains only lower level
information about how to generate language, we freeze it during task transfer. We want only the
high level ideas represented by $z$ and the predictor which receives direct
feedback to adapt to the new task. If we updated the speaker then its language
could drift given only the sparse feedback available in each new setting.
% TODO: change this claim... support it with the evidence from the experiment section

\paragraph{Adaptation Curriculum.}
As the pre-trained (stage 1) model has never had to keep track of dialog contexts beyond the first round, we fine-tune in two stages, 2.A and 2.B. In {\bf stage 2.A} we fix the Context Encoder and Question Policy parts of the planner
so the model can learn to track dialog effectively without trying
to generate better dialog at the same time. This stage takes 20 epochs
to train. Once \qbot{} learns how to track dialog we update the
entire planner in {\bf stage 2.B} for 5 epochs.\footnotemark

\footnotetext{We find 5 epochs stops training early enough to
avoid overfitting on our val set.}

==> Dialog Without Dialog NeurIPS/sections/broader_impact.tex <==
\section{Broader Impact}
\label{sec:broader_impact}

We think the main ethical aspects of this work and their consequences for society have to do with fairness. There is an open research problem around existing deep learning models often reflecting and amplifying undesirable biases that exist in society.

While visual question answering and visual dialog models do not currently work well enough to be relied on in the real world (largely because of the aforementioned proneness to bias), they could be deployed in applications where these biases could have negative impacts on fairness in the future. 
For example, visually impaired users might use these models to understand visual aspects of their world~\cite{vizwiz}. If these models are not familiar with people in certain contexts (e.g., men shopping) or are only used to interacting with certain users (e.g., native English speakers) then they might fail for some sub-groups (e.g., non-native English speakers who go shopping with men) but not others.

Our research model may be prone to biases, though it was trained on the VQAv2 dataset~\cite{vqav2}, which aimed to be more balanced than its predecessor. However, by increasing the intelligibility of generated language our work may help increase the overall interpretability of models. This may help by making bias easier to measure and providing additional avenues for correcting it.

% We think the main ethical aspects of this work and their consequences for society
% have to do with fairness and bias.
% Vision and language models are generally known to be prone to
% overfitting to dataset biases.
% These observations often point out how models do not generalize as desired,
% generating outputs because they are often correct, even though they are
% wrong in the current context.
% This same proneness to bias can emphasize undesirable societal biases
% which some datasets capture by default~\cite{men_shop,wang20}.

% While visual question answering and visual dialog models do not currently work
% well enough to be relied on in the real world (largely because of the aforementioned proneness to bias),
% they could be deployed in applications where these biases could have negative impacts on
% fairness in the future. For example,
% \begin{compactitem}[\hspace{3pt}--]
% \item
% Visually impaired users might use these models to understand visual aspects of their world~\cite{vizwiz}.
% If these models are not familiar with people in certain contexts (\eg, men shopping)
% or are only used to interacting with certain users (\eg, native English speakers)
% then they might fail for some sub-groups (\eg, non-native English speakers who go shopping with men)
% but not others.

% \item
% These models might be used to efficiently query visual surveillance systems.
% If these models tend to identify certain kinds of people with certain activities
% then they might unfairly and incorrectly highlight those individuals.
% \end{compactitem}

% Our research model does not take these factors into account, except that it was the VQAv2 dataset~\cite{vqav2},
% which aimed to be more balanced than its predecessor.
% However, by increasing the intelligibility of generated language our work may help
% increase the overall interpretability of models.
% This may help by making bias easier to measure and providing additional avenues for correcting it.

==> Dialog Without Dialog NeurIPS/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper we proposed the Dialog without Dialog (\dwd{}) task along with a model
designed to solve this task and an evaluation scheme that takes its goals into account.
The task is to perform the image guessing game, maintaining language quality without dialog level supervision.
This balance is hard to strike, but our proposed model manages to strike it.
Our model approaches this task by representing dialogs with a discrete latent variable and
carefully transfering language information via multi stage training.
While baseline models either adapt well to new tasks or maintain language
quality and intelligibility, our model is the only one to do both
according to both automated metrics and human judgements.
We hope these contributions help inspire useful dialog agents that can also interact with humans.


==> Dialog Without Dialog NeurIPS/sections/experiments.tex <==
\section{Experiments} \label{sec:experiments}

We want to show that our proposed agent can adapt to new tasks while exhibiting less linguistic drift.
In \secref{sec:experimental_settings} and \secref{sec:baselines} we start by describing
the new tasks we construct and the baselines we compare to, then
the following sections demonstrate how our model adapts while preventing drift using
qualitative examples (\secref{sec:qualitative}),
automated metrics (\secref{sec:auto_eval}),
and human judgements (\secref{sec:human-study}).
We also summarize the model ablations (\secref{sec:ablations}) detailed in the supplement.

\paragraph{Task Settings.}
\label{sec:experimental_settings}
We construct new tasks by varying four parameters of our image guessing game:
\begin{compactitem}[--]
\item \textbf{Number of Dialog Rounds.}
The number of dialog rounds $R$ is fixed at 1, 5, or 9.

\item \textbf{Pool Size.}
The number of images in a pool $P$ to 2, 4, or 9.

\item \textbf{Image Domain.}
By default we use VQA images (\ie, from COCO~\cite{LinECCV14coco}),
but we also construct pools using CUB (bird) images~\cite{cub} and
AWA (animal) images~\cite{awa2}.

\item \textbf{Pool Sampling Strategy.}
We test two ways of sampling pools of images. The Constrast sampling method,
required for pre-training (\secref{sec:stage1}),
chooses a pair of images with contrasting answers to the same question from VQAv2.
This method only works for $P=2$.
The Random sampling method chooses $P$ images at random from the images available
in the split.
\end{compactitem}
For example, consider the `VQA - 2 Contrast - 5 Round' setting. %To understand the notation in \tabref{tab:main_results} take  as an example.
These pools are constructed from 2 VQA images with the Contrast sampling strategy and dialogs are rolled out to 5 rounds.

\iffalse 
We list out specific settings below:
\begin{compactitem}
\item \textbf{VQA - 2 Contrast - 1 Round.} This is precisely the data and dialog setting from the stage one pretraining. Performance here is diagnostic for how well models can generalize just to new in-domain instances. 
\item \textbf{VQA - 2 Contrast - 5 Round.} Using the same data source as the previous setting (and stage one training), this setting extends to five rounds of dialog -- asking agent to adapt to the sequential nature of the task.
\item \textbf{VQA - 2 Random - 5 Round.} Still using VQA images, this setting provides a baseline for performance on random image pools. As there are no pre-defined contrastive contrastive pairs
\end{compactitem}
\fi


\subsection{Baselines}
\label{sec:baselines}

We compare our proposed approach to two baselines -- \textbf{\stageone{}} and \textbf{\nonvar{}} -- ablating aspects of our model that promote
adaptation to new tasks or prevent language drift.
%with a few variants of our approach to systematically study our design choice. 
The \textbf{\stageone{}} baseline is our model after the single round fully supervised pre-training.
Improvements over this model represent gains made from task based fine-tuning.
The \textbf{\nonvar{}} baseline is our model under standard encoder-decoder dialog model design choices -- \ie,
a continuous latent variable, maximum likelihood pre-training, and fine-tuning the speaker module. 
Improvements over this model represent gains made from the modifications aimed at preventing language drift described in \secref{sec:new_qbot} --
specifically, the discrete latent variable, ELBO pre-training, and frozen speaker module.

\begin{figure}[!h]\footnotesize
    \centering
    \vspace{-10pt}
    \includegraphics[width=\textwidth]{figures/Fig5.pdf}
    \vspace{-18pt}
    \caption{\footnotesize{Qualitative comparison of dialogs generated by our model with
        those generated by \nonvar{} and \stageone{} baselines. Top / middle / bottom rows are image pool from COCO / AWA / CUB images respectively. Our model is pre-trained on VQA (COCO images) and generates more intelligible questions on out-of-domain images.}}
    \vspace{-10pt}  
    \label{fig:examples}
\end{figure}


\subsection{Qualitative Results}
\label{sec:qualitative}
Figure~\ref{fig:examples} shows example outputs of the \nonvar{} and \stageone{} baselines alongside our \qbot{}
on VQA, AWA and CUB images using size 4 Randomly sampled pools and 5 rounds of dialog.
Both our model and the \nonvar{} baseline tend to guess the target image correctly,
but it is much easier to tell what the questions our model asks mean and how they might
help with guessing the target image.
On the other hand, questions from the \stageone{} baseline are clearly grounded in
the images, but they do not seem to help guess the target image and the \stageone{} baseline
indeed fails to guess correctly.
This is a pattern we will reinforce with quantitative results in \secref{sec:human-study} and \secref{sec:auto_eval}.

These examples and others we have observed suggest interesting patterns that highlight \abot{}.
Our automated \abot{} based on \cite{bottomup} does not always provide accurate answers,
limiting the questions \qbot{} can usefully ask.
When there is signal in the answers, it is not necessarily intelligible, providing an opportunity
for \qbot{}'s language to drift.


\subsection{Automated Evaluation}
\label{sec:auto_eval}

%\subsubsection{Metrics}
%\label{sec:metrics}

We consider metrics addressing both {\bf Task} performance and {\bf Language} quality.
While task performance is straightforward (did \qbot{} guess the correct target image?), language quality
is harder to measure. We describe three automated metrics here and further investigate language
quality using human evaluations in \secref{sec:human-study}.% a diverse set of five metrics including
%two that asked humans to compare questions asked by different bots.

\paragraph{Task -- Guessing Game Accuracy.}
To measure task performance so we report the accuracy of \qbot{}'s target image guess at the
final round of dialog.

\paragraph{Language -- Question Relevance via \abot{}.}
%If a generated question is not relevant to at least one pool image, then it will be very hard for humans to understand
%the questions, and thus it will be less likely that our \qbot{}
%can interact effectively with humans.
To be human understandable, the generated questions should be relevant to at least one image in the pool. We measure question relevance as the maximum question 
image relevance across the pool as measured by \abot{}, i.e., $1 - p(\texttt{Not Relevant})$. We note that this is only a proxy for actual question relevance as 
\abot{} may report \texttt{Not Relevant} erroneously if it fails to understand \qbot{}'s question; however, in practice we find \abot{} does a fair job in 
determining relevance. We also provide human relevance judgements in \secref{sec:human-study}. %\todo{Report some quantitative measure even if it is just you looking over 50 relevant vs not relevant predicted questions}

%Our modified \abot{} has a \texttt{Not Relevant} token in its vocabulary,
%so we use that to evaluate relevance. Specifically,
%the probability a question is relevant to a given image is relevance $ = 1 - p(\texttt{Not Relevant})$.
%To compute the relevance of a question to an entire pool, we simply take the max relevance over all images.

% TODO: report actual abot performance
%While our modified \abot{} is far from perfect,
%qualitatively it still does a fair job at determining when
%a question is or is not relevant to image content.
%Furthermore, its notion of relevance takes into account its own failings:
%questions which are relevant but not understood by \abot{} are
%still not useful for \qbot{} to ask, so they are counted as not relevant.


\paragraph{Language -- Fluency via Perplexity.}
To evaluate \qbot{}'s fluency, we train
an LSTM-based language model on the corpus of questions in VQA.
This allows us to evaluate the perplexity of the questions generated
by \qbot{} for dialogs on its new tasks. Lower perplexity indicates
the generated questions are similar to VQA questions in terms of syntax
and content. However, we note that questions
generated for the new tasks could have lower perplexity because they have drifted from English or because different
things must be asked for the new task, so lower perplexity
is not always better~\cite{gen_eval}.


\paragraph{Language -- Diversity via Distinct $n$-grams.}
This considers the set of all questions generated by \qbot{}
across all rounds of dialog on the val set.
It counts the number of $n$-grams in this set, $G_n$, and the number of
distinct $n$-grams in this set, $D_n$, then reports $\frac{G_n}{D_n}$
for each value of $n \in \{1, 2, 3, 4\}$.
Note that instead of normalizing by the number of words as in previous
work~\cite{dbs,li15ado}, we normalize by the number of n-grams so
that the metric represents a percentage for values of $n$ other than $n=1$.
Generative language models frequently produce safe standard outputs~\cite{dbs},
so diversity is a sign this problem is decreasing, but diversity by itself 
does not make language meaningful or useful.

%\subsubsection{Results}
%\label{sec:main_results}

\paragraph{Results.}
Table \ref{tab:main_results} presents results on our val set for our model and
baselines across the various settings described in \secref{sec:experimental_settings}.
Agents are tasked with generalizing further and further from their source language data.
Setting \texttt{A} is the same as for stage 1 pre-training.
In that same column, \texttt{B} and \texttt{C} 
require generalization to multiple rounds of dialog and Randomly sampled image pairs instead of pools sampled with the Contrast strategy.
In the right side of \tabref{tab:main_results} we continue to test generalization farther from the language source
using more images and rounds of dialog (\texttt{D}) and then using different types of images (\texttt{E} and \texttt{F}).
Our model performs well on both task performance and language quality across the different settings in terms of these
automatic evaluation metrics. Other notable findings are:
 
\begin{table}[h]
\input{result_tables/main_results_table.tex}
\caption{
%Performance of our models and baselines in different experimental settings. Starting from the first setting and moving downward, agents are tasked with generalizing further and further from their source data -- from setting \texttt{A} which mimics the human data pretraining to setting \texttt{F} where agents must carry on a nine round dialog about 9 images containing only different bird species. Our method strikes a balance between guessing game performance and interpretability where as the baseline Stage 1 model performs poorly on new tasks and the Non-Variation Continuous baseline produces divergent language (also see \tabref{tab:human_studies_fluency} and \tabref{tab:human_studies_relevance}).
Performance of our models and baselines in different experimental settings. From setting \texttt{A} to setting \texttt{F}, agents are tasked with generalizing further from the source data. Our method strikes a balance between guessing game performance and interpretability.
}
\vspace{-10pt}
\label{tab:main_results}
\end{table}

\paragraph{Ours \vs \stageone{}.} To understand the relative importance of the proposed stage 2 training which transferring to dialog for DwD task, we compared the task accuracy of our model with that of \stageone{}. In setting, \texttt{A} which matches the training regime, our model outperforms \stageone{} by 9\% (\texttt{A3} \vs \texttt{A1}) on task performance. As the tasks differ in settings B-F, we see further gains with our model consistently outperforming \stageone{} by 20-38\%. Despite these gains, our model maintains similar language perplexity, A-bot relevance, and diversity. 

\paragraph{Ours \vs \nonvar{}.} Our discrete latent variable, variational pre-training objective, and fixed speaker play an important role in avoiding language drift. Compared to the \nonvar{} model without these techniques, our model achieves over 4x (\texttt{A2} / \texttt{A3}) lower perplexity and 10-53\% better A-bot Relevance. Our model also improves in averaged accuracy, which means more interpretable language also improves the task performance. Note that \nonvar{} has 2-100x higher diversity compared to our model, which is consistent with the gibberish we observe from that model (\eg, in \figref{fig:examples}) and further suggests its language is drifting away from English.

\paragraph{Results from Game Variations.} We consider the following variations on the game:
\begin{compactitem}[--]
\item \textbf{Dialog Rounds.} Longer dialogs (more rounds) achieve better accuracy (A3 vs B3). 

\item \textbf{Pool Sampling Strategy.} As expected, Random pools are easier compared to Contrast pools (B3 vs C3 accuracy), however language fluency and
relevance drop on the Random pools (B3 vs C3 perplexity and a-bot relevance).  

\item \textbf{Image Source.} CUB and AWA pools are harder compared to COCO image domain (D3 vs E3 vs F3). Surprisingly, our models maintains similar perplexity and high a-bot relevance even on these out-of-domain image pools. The \stageone{} and \nonvar{} baselines generalize poorly to these different image domains -- reporting task accuracies nearly half our model performance.

\end{compactitem}



\subsection{Human Studies}
\label{sec:human-study}

We also evaluate our models by asking if humans can understand \qbot{}'s language.
Specifically, we use workers (turkers) on Amazon Mechanical Turk to evaluate the relevance, fluency,
and task performance of our models. Section \suppSectionHumanStudies{} of the supplement details these studies,
but we briefly summarize the results here.

Turkers from Amazon's Mechanical Turk considered the questions from our model more relevant to the image pool than those
from the \nonvar{} model and about equally as relevant as the \stageone{} model's questions.
Similarly, they considered our model's questions more fluent than the \nonvar{} model questions and equally
as fluent as the \stageone{} model's questions.
However, when we used used turkers to answer \qbot{}'s questions
-- replacing the automated \abot{} -- our \qbot{} was able to guess the correct image 69\% of the time while
the \nonvar{} only achieved 45\% accuracy and the \stageone{} model achieved 23\% accuracy.
This again confirms that our model can adapt to new tasks with minimal
sacrifice to language quality.



\subsection{Model Ablations}
\label{sec:ablations}

We investigate the impact of our modelling choices from \secref{sec:new_qbot}
by ablating these choices in Section \suppSectionAblations{} of the supplement, summarizing the
results here.
The choice of discrete instead of continuous $z^r$ helps maintain language
quality, as does the use of variational (ELBO) pre-training instead of maximum likelihood.
Surprisingly, the ELBO loss probably has more impact than the discreteness of $z^r$.
Fixing the speaker module during stage 2 also had a minor role in discouraging language drift.
Finally, we find that improvements in task performance are due more to learning to track
the dialog in stage 2.A than they are due to asking more discriminative questions.

==> Dialog Without Dialog NeurIPS/sections/intro.tex <==
\section{Introduction}
One goal of AI is to enable humans and computers to
communicate naturally with each other in grounded language
to achieve a collaborative objective. Recently the community has studied 
goal oriented dialog, where agents communicate
for tasks like booking a flight or searching for images \cite{miller2017parlai}.

A popular approach to these tasks has been to observe humans engaging 
in dialogs like the ones we would like to automate and then train agents 
to mimic these human dialogs~\cite{visdial_rl,deal_or_no_deal}.
Mimicking human dialogs allows agents to generate intelligible language (\ie, 
meaningful English, not gibberish). However, these models are typically fragile and generalize poorly to new tasks. 
As such, each new task requires collecting new human dialogs, which is a laborious 
and costly process often requiring many iterations
before high quality dialogs are elicited \cite{visdial, guesswhat}. 

A promising alternative is to use goal completion as a supervisory signal
to adapt agents to new tasks.
Specifically, this is realized by pre-training dialog agents via human dialog supervision on one
task and then fine-tuning them on a new task by rewarding the agents
for solving the task regardless of the dialog's content. This approach can indeed 
improve task performance, but language quality suffers 
even for similar tasks. It tends to drifts from human language, becoming ungrammatical 
and loosing human intelligible semantics -- sometimes even turning into unintelligible code.
Such code may allow communication with other bots, but is largely incomprehensible to humans. 
This trade off between task performance and language drift has been observed in prior dialog work~\cite{visdial_rl,deal_or_no_deal}.
 
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/Fig1.pdf}
    \vspace{-15pt}
    \caption{An example of \textit{Dialog without Dialog} (DwD) task: (Left) We pre-train questioner agent (\qbot{} in green) that can discriminate
    between pairs of images by mimicking questions from VQAv2 \cite{vqav2}. 
    (Right) \qbot{} needs to generate a sequence of discriminative questions (a dialog) to identify the secret image that \abot{} picked. Note that the language supervision is not available, thus we can only fine-tune \qbot{} with task performance. In DwD, we can test \qbot{} generalization ability by varying dialog length, pool size and image domain.
    % These new settings include images from different domains, 
    % In these two (top and bottom) single round dialogs we train our questioner to ask questions that can discriminate
    % between pairs of images by mimicking questions known to be discriminative from the VQAv2 dataset.
    % (Right) Our proposed model generalizes to new settings where language supervision is not available.
    % These new settings may include images from different domains (like the birds seen here),
    % and they require agents to discriminate between more than 2 images, thus necessitating multiple rounds of dialog.
    % Furthermore, our model generalizes in two senses: 1) it can discriminate between images in these
    % new settings, and 2) it continues to use language humans can understand
    % instead of exhibiting the language drift seen in other work.
    }
    \vspace{-10pt}
    \label{fig:guesswhich}
\end{figure}
 
The goal of this paper is to 
develop visually grounded dialog models that can adapt to new tasks while exhibiting less linguistic drift, thereby reducing
the need to 
collect new data for the new tasks.
% pick task performance or language quality.
To test this we consider an image guessing game demonstrated in \figref{fig:guesswhich} (right).
In each episode, one agent (\abot{} in red) secretly selects a target image $y$ (starred) from a pool of images. The other agent (\qbot{} in green) must identify this image by asking questions
for \abot{} to answer in a dialog. To succeed, \qbot{} needs to understand the
image pool, generate discriminative questions, and interpret the answers \abot{}
provides to identify %
%\abot{}'s selected image \jl{(in the dashed green box). }
the secret image. 
%reason we use this game. 
The image guessing game provides the agent with a goal, and we can test \qbot{} generalization ability by varying dialog length, pool size and image domain.

%\jl{I felt there is something missing here. We directly give the contribution without any context. Is that fine? }

\paragraph{Contribution 1.}
We propose the \textit{Dialog without Dialog} (\dwd{}) task, which requires a \qbot{} to perform our image
guessing game without dialog level language supervision.
%
%In \dwd{}, \qbot{} is trained with visual question answering data, but must adapt to multi-round image-discriminative dialogs about pools of new images -- including those from new domains or from large pools.
%
As shown in in \figref{fig:guesswhich} (left),  \qbot{} in this setting first learns to ask questions to identify the secret image by mimicking single-round human-annotated visual questions. For the dialog task (right), no human dialogs are available so \qbot{} can only be supervised by its image guessing performance. To measure task performance and language drift in increasingly out-of-distribution settings we consider varied pool sizes and take pool images from diverse image sources (\eg close-up bird images).




%Then, as shown in \figref{fig:guesswhich} (right), \qbot{} needs to identify the secret image from a new image pool by engaging in dialogs with \abot{}. Note that the image pool may vary in size and image domain and we do not have dialog annotations. \qbot{} can only be supervised by the task performance. 
% Then we introduce different image pools\footnotemark{} and \qbot{}  
% Note that we do not have dialog annotations,
 %Because the data used during pre-training requires question level supervision, it can only
 %contain pools of 2 images from the VQAv2~\cite{vqav2} dataset specifically constructed to provide a fully informative answer in only one round of dialog.
 %Guessing game performance on the new pools allows us to test adaptation to new tasks, while the lack of question supervision allows us to test language drift.

% \footnotetext{
% These pools differ from the pre-training pools because they have
% more than 2 images that are randomly sampled (not determined by constrasting pairs from VQAv2)
% and require multiple questions (a dialog) to guess the target image.
% We test pools of animal and bird images instead of the COCO images from VQAv2.}

\paragraph{Contribution 2.}
We propose a \qbot{} architecture for the \dwd{} task
that decomposes question intent from the words used to express that intent.
% \jl{We propose a \qbot{} architecture for the \dwd{} task that disentangles `how to ask' and `what to ask'.
%
We model the question intent by introducing a discrete latent representation 
that is the only input to the language decoder. 
% We pair this with a learning curriculum that adapts \qbot{}
% to dialog in stages -- first learning to follow the dialog and then to generate new questions.
We further pair this with a \textit{pre-train then fine-tune} learning approach that teaches \qbot{} how to ask visual questions from VQA during pre-training and `what to ask' during fine-tuning for visual dialogs.

\paragraph{Contribution 3.}
We measure \qbot{}'s ability to adapt to new tasks and maintain language
quality.
Task performance is measured with both automatic and human answerers
while language quality is measured using three automated metrics
and two human judgement based metrics.
Our results show the proposed \qbot{} both adapts to new tasks better than
a baseline chosen for language quality and maintains language quality better
than a baseline optimized for just task performance.

%In \secref{sec:guessgame} we describe our image guessing game in more detail, then we
%build our \qbot{} for \dwd{} in \secref{sec:dwd}.
%\secref{sec:experiments} evaluates this model, 
%\secref{sec:rel_work} relates our approach to previous work,
%and \secref{sec:conclusion} summarizes our findings.


==> Dialog Without Dialog NeurIPS/sections/rel_work.tex <==
\section{Related Work}
\label{sec:rel_work}

Our interest comes from language drift problems encountered when using models comparable to
the \stageone{} baseline. In \cite{deal_or_no_deal} a dataset
is collected with question supervision then fine-tuning is used in
an attempt to increase task performance, but the resulting utterances
are unintelligible. Similarly, \cite{visdial_rl} takes a very careful
approach to fine-tuning for task performance but finds that
language also diverges, becoming difficult for humans to understand.
Neither approach uses a discrete latent variables or a multi stage training curriculum, as in our proposed model.
Furthermore, these models need to be adapted to work in our new setting, and doing so would yield
models very similar to our \nonvar{} baseline.

More recently, \cite{drift_emnlp19} observe language drift in a translation game from French to German.
They reduce drift by supervising communications between agents with auxiliary translations to English and grounding in images.
This setting is somewhat different than ours since grounding is directly necessary to solve our task.
The approach also requires direct supervision on the communication channel, which is not practical
for a multiple round dialog game like ours.

We used a visual reference game to study question generation,
improving the quality of generated language using concepts related to latent action spaces.
Some works like \cite{lba} and \cite{visual_curiosity} also aim
to ask visual questions with limited question supervision.
Other works represent dialog using latent action spaces~\cite{rethink_zhao, zhao_unsup, zero_shot_zhao, yarats2017hierarchical, wen2017latent, serban2016piecewise, yarats2017hierarchical, hu2019hierarchical, kang2019recommendation, serban2017hierarchical, williams2017hybrid}. 
Finally, reference games are generally popular for studying language~\cite{lewis,guesswhat,visdial_eval}.
Section \suppSectionRelWork{} of the supplement describes the relationship between our approach
and these works in more detail.

==> Dialog Without Dialog NeurIPS/sty/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> result_tables/ablations.tex <==
{\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr}
\toprule
& Accuracy & Perplexity & Relevance & Diversity \\
\midrule
DWD (Ours)           &     0.81 &      2.57 &         0.89 &        0.86 \\
Fine Decoder         &     0.82 &      2.54 &         0.85 &        0.59 \\
Parallel Speaker     &     0.78 &      2.60 &         0.88 &        0.73 \\
Stage 1              &     0.72 &      2.60 &         0.91 &        0.48 \\
Stage 2.A            &     0.80 &      2.59 &         0.89 &        0.81 \\
Stage 2.B (Skip 2.A) &     0.80 &      2.53 &         0.85 &        0.62 \\
\bottomrule
\end{tabular}
}
}

==> result_tables/human_interactive.tex <==




{
\newcommand{\num}[1]{\texttt{\footnotesize #1}}

\resizebox{\columnwidth}{!}{
\begin{tabular}{l c c c c c}
\toprule
            & Accuracy \\
Round       & 1         & 2         & 3         & 4         & 5 \\
\midrule
\stageone{} & 20.8\%	&  25.0\%	&  22.9\%	&  35.4\%	&  22.9\% \\
\nonvar{}   & 26.5\%	&  53.1\%	&  51.0\%	&  46.9\%	&  44.9\% \\
\ours{}     & 18.4\%	&  61.2\%	&  53.1\%	&  65.3\%	&  69.4\%
\bottomrule
\end{tabular}
}

==> result_tables/mturk_question_comparison.tex <==
{\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr}
\toprule
                       & Neither & \stageone{} & \nonvar{} & \ours{}   \\
\midrule                          
\stageone{} vs \nonvar{} &  31.7\% &  48.1\%   &  20.2\%   &  --     \\
\stageone{} vs \ours{}     &  49.0\% &  26.2\%   &  --       &  24.8\% \\
\nonvar{} vs \ours{}     &  32.7\% &  --       &  17.9\%   &  49.4\% \\
\midrule
\stageone{} vs \nonvar{} &  19.6\% &  48.8\%   &  31.7\%   &  --     \\
\stageone{} vs \ours{}     &  25.0\% &  38.4\%   &  --       &  36.6\% \\
\nonvar{} vs \ours{}     &  22.0\% &  --       &  30.2\%   &  47.8\% \\
\bottomrule
\end{tabular}
}
}

==> result_tables/mturk_question_comparison_fluency.tex <==
%% fluency raw counts
%\begin{tabular}{lrrrr}
%\toprule
%choice\_name &  baseline &  neither &   ours &  stage 1 \\
%exp\_pair                    &           &          &        &          \\
%\midrule
%exp15.0.1.0.0\_exp19.2.1.0.4 &     182.0 &    285.0 &    NaN &    433.0 \\ 900
%exp15.0.1.0.0\_exp20.2.2.0   &       NaN &    441.0 &  223.0 &    236.0 \\ 900
%exp19.2.1.0.4\_exp20.2.2.0   &     161.0 &    294.0 &  445.0 &      NaN \\ 900
%\bottomrule
%\end{tabular}


{\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr}
\toprule
                       & Neither & \stageone{} & \nonvar{} & \ours{}   \\
\midrule                          
\stageone{} vs \nonvar{} &  31.7\% &  48.1\%   &  20.2\%   &  --     \\
\stageone{} vs \ours{}     &  49.0\% &  26.2\%   &  --       &  24.8\% \\
\nonvar{} vs \ours{}     &  32.7\% &  --       &  17.9\%   &  49.4\% \\
\bottomrule
\end{tabular}
}
}

==> result_tables/mturk_question_comparison_grounding.tex <==
%% grounding raw counts
%\begin{tabular}{lrrrr}
%\toprule
%choice\_name &  baseline &  neither &   ours &  stage 1 \\
%exp\_pair                    &           &          &        &          \\
%\midrule
%exp15.0.1.0.0\_exp19.2.1.0.4 &     285.0 &    176.0 &    NaN &    439.0 \\ 900
%exp15.0.1.0.0\_exp20.2.2.0   &       NaN &    225.0 &  329.0 &    346.0 \\ 900
%exp19.2.1.0.4\_exp20.2.2.0   &     272.0 &    198.0 &  430.0 &      NaN \\ 900
%\bottomrule
%\end{tabular}




{\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr}
\toprule
                       & Neither & \stageone{} & \nonvar{} & \ours{}   \\
\midrule                          
\stageone{} vs \nonvar{} &  19.6\% &  48.8\%   &  31.7\%   &  --     \\
\stageone{} vs \ours{}     &  25.0\% &  38.4\%   &  --       &  36.6\% \\
\nonvar{} vs \ours{}     &  22.0\% &  --       &  30.2\%   &  47.8\% \\
\bottomrule
\end{tabular}
}
}

==> result_tables/vartype_comparison.tex <==
{\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrr}
\toprule
& Accuracy & Perplexity & Relevance & Diversity \\
\midrule
Cont Stage 2.B         &     0.75 &      2.45 &         0.66 &        0.23 \\
DWD (Ours)             &     0.81 &      2.57 &         0.89 &        0.86 \\
Non-Var Cont Stage 2.B &     0.78 &      4.27 &         0.83 &        4.33 \\
\bottomrule
\end{tabular}
}
}

==> sty/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

